Reinforcement Learning for Adaptive MCMC

An informal observation, made by several authors, is that the adaptive design of a Markov transition kernel has the flavour of a reinforcement learning task. Yet, to-date it has remained unclear how to actually exploit modern reinforcement learning technologies for adaptive MCMC. The aim of this paper is to set out a general framework, called Reinforcement Learning Metropolis--Hastings, that is theoretically supported and empirically validated. Our principal focus is on learning fast-mixing Metropolis--Hastings transition kernels, which we cast as deterministic policies and optimise via a policy gradient. Control of the learning rate provably ensures conditions for ergodicity are satisfied. The methodology is used to construct a gradient-free sampler that out-performs a popular gradient-free adaptive Metropolis--Hastings algorithm on $\approx 90 \%$ of tasks in the PosteriorDB benchmark.

==> figures/demo/mixture_gaussian_1D/RL_reward_demo_tikz.tex <==
\begin{tikzpicture}
    \begin{axis}[
        xlabel={$n$},
        ylabel={$r_{n}$},
        width=\linewidth,
        height=\linewidth,
        tick label style={font=\tiny},
        label style={font=\scriptsize},
        % axis line style={draw=none},
        tick style={draw=none},
        scale only axis,
        enlargelimits=false,
        clip=false,
        % xlabel style={at={(axis description cs:0.5,0.02)},anchor=north},
        % ylabel style={at={(axis description cs:0.02,0.5)},anchor=south},
        % xlabel style={yshift=-0.5em},
        % ylabel style={yshift=+0.5em},
    ]
    \addplot[
        mark=none,
        color={rgb,1:red,0.4078;green,0.4078;blue,0.5373}
    ] coordinates {
        (0, -3.0292597658250315)
        (500, -6.930080603462622)
        (1000, -11.572366534593261)
        (1500, -12.418876645522413)
        (2000, -12.44022882463031)
        (2500, -12.558006753992375)
        (3000, -9.617184110520945)
        (3500, -5.752606359650183)
        (4000, -5.449366764644949)
        (4500, -5.288662713374647)
        (5000, -22.819241211787496)
        (5500, -41.18762793312521)
        (6000, -41.28846465622597)
        (6500, -41.03388854150275)
        (7000, -40.57347784305241)
        (7500, -22.958159553613303)
        (8000, -5.014733339511452)
        (8500, -5.5118851259714825)
        (9000, -6.158230309820825)
        (9500, -6.293686406843876)
        (10000, -5.60845870354759)
        (10500, -5.0858051987295445)
        (11000, -4.5837813643977725)
        (11500, -5.908655134005866)
        (12000, -13.238975456738315)
        (12500, -14.189750354761282)
        (13000, -13.821891921356022)
        (13500, -13.473710707029849)
        (14000, -11.32405648018771)
        (14500, -3.727739582070318)
        (15000, -2.794610536400911)
        (15500, -2.899811538902789)
        (16000, -2.7120860839313132)
        (16500, -2.9053768973335026)
        (17000, -2.390599426121915)
        (17500, -2.386464283627884)
        (18000, -1.9563269813692954)
        (18500, -1.4139790713433191)
        (19000, -0.3654973849768375)
        (19500, 0.1394322985728222)
        (20000, 1.04832372270804)
        (20500, 1.717000318085639)
        (21000, 1.952539921624949)
        (21500, 1.8384138195993678)
        (22000, 2.1387455000777993)
        (22500, 2.0887117350775215)
        (23000, 1.7646374182516897)
        (23500, 1.812241227930511)
        (24000, 1.8209797404944248)
        (24500, 1.587133873963876)
        (25000, 1.3579301443984413)
        (25500, 1.5272055675260567)
        (26000, 1.5958558131496408)
        (26500, 1.807609810939105)
        (27000, 2.056010831017492)
        (27500, 2.5787033517166664)
        (28000, 2.9000005523688985)
        (28500, 3.0182683835245623)
        (29000, 3.24420332486612)
        (29500, 3.3709922755525796)
        (30000, 3.368220604042677)
        (30500, 3.4274734261590893)
        (31000, 3.4328819690880668)
        (31500, 3.514914244294329)
        (32000, 3.40691254285994)
        (32500, 3.471944060715816)
        (33000, 3.3546945635931147)
        (33500, 3.402306553335032)
        (34000, 3.164828332917301)
        (34500, 3.261170783885429)
        (35000, 3.1706487562336827)
        (35500, 3.0587764663776933)
        (36000, 3.072584183001864)
        (36500, 3.2411368670958716)
        (37000, 3.2251022257656077)
        (37500, 3.2772185583173212)
        (38000, 3.5696192215357545)
        (38500, 3.5824745395120177)
        (39000, 3.59933269744837)
        (39500, 3.604478628714875)
        (40000, 3.5820435856163195)
        (40500, 3.556225398064021)
        (41000, 3.5630338842528393)
        (41500, 3.682257608537779)
        (42000, 3.5747400435554906)
        (42500, 3.6159958094948497)
        (43000, 3.6558820099170237)
        (43500, 3.479357995238517)
        (44000, 3.478392615168525)
        (44500, 3.6489784133866894)
        (45000, 3.7105314356965193)
        (45500, 3.689495277281134)
        (46000, 3.8814224854543733)
        (46500, 3.7035714248269898)
        (47000, 3.6408485561501793)
        (47500, 3.6327998086136772)
        (48000, 3.6648106702052123)
        (48500, 3.643086319204975)
        (49000, 3.8290894679737857)
        (49500, 3.7403420759689956)
        (50000, 3.7625166928459484)
        (50500, 3.7127222789434047)
        (51000, 3.682476398895299)
        (51500, 3.5874482163327626)
        (52000, 3.7914625673066786)
        (52500, 3.794179144301695)
        (53000, 3.835217195154242)
        (53500, 3.749815642733926)
        (54000, 3.862119869209708)
        (54500, 3.830450421575285)
        (55000, 3.8680358363891307)
        (55500, 3.823331345170809)
        (56000, 3.961868947115323)
        (56500, 3.924635978667924)
        (57000, 3.878957795310222)
        (57500, 3.8811431786979167)
        (58000, 3.9087623630755446)
        (58500, 3.8467604620360643)
        (59000, 3.833311281059544)
        (59500, 3.7902225821534716)
        (60000, 3.721785235066825)
        (60500, 3.7294671988726242)
        (61000, 3.7781816732254088)
        (61500, 3.8115015024852603)
        (62000, 3.7926111414357986)
        (62500, 3.831587190792759)
        (63000, 3.814130407422743)
        (63500, 3.8222721142830927)
        (64000, 3.7688927009530873)
        (64500, 3.810359695691253)
        (65000, 3.7503751086240764)
        (65500, 3.748788033210391)
        (66000, 3.7272161652857614)
        (66500, 3.7736884778941295)
        (67000, 3.831781469413852)
        (67500, 3.9070069128041043)
        (68000, 3.920064533134665)
        (68500, 3.945338783887231)
        (69000, 3.1613676301102718)
        (69500, 2.3587500951120344)
    };
    \end{axis}
\end{tikzpicture}


==> reward_plots.tex <==
\figureSeriesHere{%
\label{fig: full posterior db reward}

\protect\solidrlline \textsc{RL-MCMC}
\protect\solidamline \textsc{VA-MCMC}
\protect\solidnutsline \textsc{NUTS}
\protect\solidmalaline \textsc{MALA}

}{%
\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/earnings-earn_height_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/earnings-log10earn_height_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/earnings-logearn_height_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/gp_pois_regr-gp_regr_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/kidiq-kidscore_momhs_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/kidiq-kidscore_momiq_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/kilpisjarvi_mod-kilpisjarvi_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/mesquite-logmesquite_logvolume_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/arma-arma11_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/earnings-logearn_height_male_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/earnings-logearn_logheight_male_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/garch-garch11_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/hmm_example-hmm_example_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/kidiq-kidscore_momhsiq_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/earnings-logearn_interaction_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/earnings-logearn_interaction_z_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/kidiq_with_mom_work-kidscore_interaction_c_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/kidiq_with_mom_work-kidscore_interaction_c2_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/kidiq_with_mom_work-kidscore_interaction_z_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/kidiq_with_mom_work-kidscore_mom_work_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/kidiq-kidscore_interaction_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/low_dim_gauss_mix-low_dim_gauss_mix_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/mesquite-logmesquite_logva_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/bball_drive_event_0-hmm_drive_0_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/bball_drive_event_1-hmm_drive_1_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/sblrc-blr_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/sblri-blr_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/arK-arK_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/mesquite-logmesquite_logvash_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/hudson_lynx_hare-lotka_volterra_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/mesquite-logmesquite_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/mesquite-logmesquite_logvas_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/mesquite-mesquite_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/eight_schools-eight_schools_centered_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/eight_schools-eight_schools_noncentered_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/nes1972-nes_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/nes1976-nes_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/nes1980-nes_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/nes1984-nes_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/nes1988-nes_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/nes1992-nes_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/nes1996-nes_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/nes2000-nes_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/gp_pois_regr-gp_pois_regr_reward.pdf}}%
}

\figureSeriesRow{%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/diamonds-diamonds_reward.pdf}}%
\figureSeriesElement{}{\includegraphics[width = 0.45\textwidth]{figures/reward/mcycle_gp-accel_gp_reward.pdf}}%
}
}%
